A Metalearning Approach for Physics-Informed Neural Networks (PINNs): Application to Parameterized PDEs

Physics-informed neural networks (PINNs) as a means of discretizing partial differential equations (PDEs) are garnering much attention in the Computational Science and Engineering (CS&E) world. At least two challenges exist for PINNs at present: an understanding of accuracy and convergence characteristics with respect to tunable parameters and identification of optimization strategies that make PINNs as efficient as other computational science tools. The cost of PINNs training remains a major challenge of Physics-informed Machine Learning (PiML) - and, in fact, machine learning (ML) in general. This paper is meant to move towards addressing the latter through the study of PINNs on new tasks, for which parameterized PDEs provides a good testbed application as tasks can be easily defined in this context. Following the ML world, we introduce metalearning of PINNs with application to parameterized PDEs. By introducing metalearning and transfer learning concepts, we can greatly accelerate the PINNs optimization process. We present a survey of model-agnostic metalearning, and then discuss our model-aware metalearning applied to PINNs as well as implementation considerations and algorithmic complexity. We then test our approach on various canonical forward parameterized PDEs that have been presented in the emerging PINNs literature.

==> Methods.tex <==
%
\section{Methods}
\label{sec:methods}

In this section, we present two categories of methods within the CS\&E world
often applied to parameterized PDE reduced-order modeling:  statistical methods for regression and numerical methods for approximation.  We only select exemplars from both lists for our study; we acknowledge that many more methods exist.  However, we hold that these five methods help give sufficient breadth of application and insight to motivate PINNs metalearning.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Statistical Methods for Regression}

%{\bf SHANDIAN: add review of two ML methods Michael should use for %compariso.}

Gaussian processes (GPs) are powerful statistic regression models. Due to their nonparametric Bayesian nature~\cite{Rasmussen06GP}, GPs can automatically capture the complexity of the functions underlying the data, and quantify the predictive uncertainty via a closed form (\ie Gaussian). The standard GP learns a single-output stochastic process $f: \mathbb{R}^m\rightarrow \mathbb{R}$ from the training data  $\Dcal = \{(\bxi_1, y_1), \ldots, (\bxi_K, y_K)\}$ where each $\bxi_k$ is an input vector and $\bXi = (\bxi_1,...,\bxi_K)$. The function values $\f = (f(\bxi_1), \ldots, f(\bxi_K))$ are assumed to follow a multivariate Gaussian distribution --- the finite projection of a Gaussian process $\N$ on the training inputs  --- $p(\f| \bXi) = \N(\f|\bmu, \bSigma)$, where $\bmu$ are the mean function values of every input and usually set to $\0$, and the covariance matrix
\begin{linenomath}\begin{align*}
\bSigma = 
\begin{pmatrix} 
\kappa(\bxi_1, \bxi_1)  & \cdots & \kappa(\bxi_1, \bxi_K) \\
\vdots & \ddots & \vdots \\
\kappa(\bxi_K, \bxi_1) & \cdots & \kappa(\bxi_K, \bxi_K)
\end{pmatrix}
\end{align*}\end{linenomath}
where $\kappa$ is a kernel function of the input vectors. The observed outputs $\y$ are assumed to be sampled from a noisy model, \eg $p(\y|\f) = \N(\y|\f, \tau\I)$. Integrating out $\f$, we obtain the marginal likelihood $p(\y|\bXi) = \N(\y|\0, \bSigma + \tau\I)$. Computational estimation of kernel parameters and the noise variance $\tau$ is frequently achieved via maximum likelihood estimation. %We can maximize the likelihood to estimate the kernel parameters and noise variance $\tau$. 

To predict the output for a test input $\bxi^*$, we use the conditional Gaussian distribution, since the test and training outputs jointly follow a multivariate Gaussian distribution. 
\begin{linenomath}\begin{align*}
\textrm{We have } & \, p\big(f(\bxi^*)|\bxi^*, \bXi,\y\big) = \N\big(f^* | \alpha(\bxi^*), \beta(\bxi^*)\big) \\ \textrm{where } & \, \alpha(\bxi^*) = \kappa_{*}^\top (\bSigma + \tau^{-1} \I)^{-1}\y, \\ & \beta(\x^*) = \kappa(\bxi^*, \bxi^*) - \kappa_{*}^\top(\bSigma + \tau^{-1}\I)^{-1}\kappa_{*}, \\ & \, \kappa_{*} = [\kappa(\bxi^*, \bxi_1), \ldots, \kappa(\bxi^*, \bxi_K)]^\top.
\end{align*}\end{linenomath}
In particular, we use the mean of $p\big(f(\bxi^*)|\bxi^*, \bXi,\y\big)$ as the predictor at $\bxi^*$. These methods are implemented with GPyTorch \citep{gpytorch}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Multi-task Gaussian Process Modeling}
%\an{I suggest putting this section before the previous one; seems to flow better that way.}
Many tasks  require learning a function with multiple output.\footnote{Task here is used differently than in the metalearning section. We use the nomenclature of the GP field here.} A classical multi-output regression framework is multi-task GP~\cite{williams2007multi}. It models the outputs of all the tasks as a single GP, where the kernel function between arbitrary two outputs is defined as 
\begin{linenomath}\begin{align}
	g([\bxi_1, t_1], [\bxi_2, t_2]) = \kappa(\bxi_1, \bxi_2) \cdot s_{t_1 t_2},
\end{align}\end{linenomath}
where $\bxi_1, \bxi_2$ are the inputs and $t_1, t_2$ are the task indices, $\kappa(\cdot, \cdot)$ is a kernel function of the inputs, and $s_{t_1t_2}$ is the task similarity between $t_1$ and $t_2$. The training is the same as the standard GP. However, we need to estimate not only the parameters of $\kappa(\cdot, \cdot)$, but also the similarity values between each pair of tasks $\{s_{t_1t_2}\}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Linear Method of Coregularization (LMC)}

%PCA-GP~\citep{higdon2008computer}, the popular LMC-based GP model for high-dimensional simulation data via principal component analysis (PCA) ??

Another successful multi-output regression model is  the Linear Model of Coregionalization (LMC)~\cite{journel1978mining}, which assumes the outputs are a linear combination of a set of basis vectors weighted by independent random functions. We introduce $Q$ bases $\B = [\b_1, \ldots, \b_Q]^\top$ and model a $M_{\ell}$-dimensional vector function by %$\f(\x)=[f_1(\x), \ldots, f_d(\x)]^\top$ by $\f(\x) = \sum_{k=1}^K w_k(\x) \b_k = \B^\top \w(\x)$
\begin{linenomath}\begin{align}
	\hat{\underline{w}}(\bxi) = \sum_{q=1}^{Q} \b_q c_q(\bxi) = \B^\top \c(\bxi) \label{eq:LMC}
\end{align}\end{linenomath}
where $Q$ is often chosen to be much smaller than $M_{\ell}$, and the random weight functions $\c(\bxi) = [c_1(\bxi), \ldots, c_Q(\bxi)]^\top$ are sampled from independent GPs. 
%\an{Is $d$ the right letter here? Or $M_{\ell}$?}
In spite of a linear structure, the outputs $\hat{\underline{w}}$ are still nonlinear to the input $\bxi$ due to the nonlinearity of the weight functions. LMC can easily scale up to a large number of outputs: once the bases $\B$ are identified, we only need to estimate a small number of GP models ($Q \ll M_{\ell}$). For example, we can perform PCA on the training outputs to find the bases, and use the singular values as the outputs to train the weight functions. This is also referred to as PCA-GP~\cite{higdon2008computer}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Numerical Approximation Methods for Regression}

We describe here common strategies in the numerical approximation community for building emulators of the form \eqref{eq:linear-approx} from data. We choose to focus on three different types of approaches: First we build approximations via cubic spline interpolants when $\bxi$ is one or two dimensional. The second class of methods use ``meshless" radial basis function (RBF) methods with various kernels. The third class of methods are polynomial approximation schemes using least squares approximation.

We briefly describe these approaches in each section below, focusing on specifying how the coefficients $\b_k$ and basis functions $c_k(\bxi)$ in \eqref{eq:linear-approx} are chosen and computed. In all the methods, we assume availability of data $\underbar{w}(\bxi_j)$ (i.e., trained PINNs network parameters) on a discrete sampling $\{\bxi_i\}_{i=1}^{K}$. We will specify how this grid is chosen in each section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Cubic Spline Interpolation}
\label{ssec:spline}
Univariate cubic splines are smooth interpolants of data \cite{boor_practical_1978}. More precisely, with $\left(\bxi_i\right)_{i=1}^{K}$ an ordered set of points from a Latin Hypercube Sampling (LHS) design \cite{lemieux_monte_2009} on the one-dimensional interval $\mathcal{X}$, then a cubic spline approach builds the approximation $\hat{\underbar{w}}$ in \eqref{eq:linear-approx} as a piecewise cubic function, where $\hat{\underbar{w}}$ is a cubic polynomial on each interval $[\bxi_j, \bxi_{j+1}]$, and is continuously differentiable at each $\bxi_j$. One can build such an approximation in terms of divided differences of the data $\underbar{w}(\bxi_j)$, so that the coefficients $\b_k$ are linear in this data. The basis functions $c_k(\bxi)$ are then piecewise cubic polynomials. This is implemented with the SciPy package functions scipy.interpolate.UniveriateSpline and scipy.interpolate.SmoothBivariateSpline \citep{2020SciPy-NMeth}. The bivariate case does not require a tensoral grid therefore we can use it with our sampling methods with the implemtation caveat that $K \geq (x_{deg}+1)*(y_{deg}+1)$ which in the cubic spline case is $K \geq 16$. Additionally, we use the default function parameters.

%\an{What spline method do you use? You have 2D results, but splines of this type typically only work in 1D unless you have a tensorial grid.}

%\michael{Using the functions scipy.interpolate.UnivariateSpline and  scipy.interpolate.SmoothBivariateSpline, only limitation is that for the bivariate method the number of points should be at least (degree of spline in x + 1)*(degree of spline in y + 1) so for most hypercross sampling sizes this allows for cubic (degree 3)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Radial Basis Function (RBF) Interpolation}

RBF approximations build the emulator $\hat{\underbar{w}}$ in \eqref{eq:linear-approx} using shifted kernels as basis functions,
\begin{linenomath}\begin{align*}
  c_k(\bxi) = \kappa(\bxi, \bxi_k),
\end{align*}\end{linenomath}
and the coefficients $\b_k$ are chosen by enforcing interpolation of $\hat{\underbar{w}}$ on the data points \cite{fasshauer_meshfree_2007}. We again choose the parametric grid as an LHS design, and employ three different types of commonly used kernels:
\begin{linenomath}\begin{align*}
  \kappa(\bxi, \boldsymbol{\zeta}) &= r^3, & \textrm{(Cubic)} \\
  \kappa(\bxi, \boldsymbol{\zeta}) &= \exp\left(-\left(\frac{r}{\tau}\right)^2\right), & \textrm{(Gaussian)}\\
  \kappa(\bxi, \boldsymbol{\zeta}) &= \sqrt{\left(\frac{r}{\tau}\right)^2 + 1} , & \textrm{(Multiquadric)}
\end{align*}\end{linenomath}
where $r = \left\| \bxi - \boldsymbol{\zeta} \right\|_2$ is the Euclidean distance between the inputs $\bxi$ and $\boldsymbol{\zeta}$, and $\tau$ is a tunable parameter, which we choose as the average pairwise distance between grid points. 
%\an{Is this how you choose $\tau$?}

We use interpolative RBF approximations, which enforce \eqref{eq:linear-approx} at every data point. Such RBF approximations are closely related to GP statistical models: an RBF approximation equals the mean of a GP approximation built from the same kernel, with zero nugget at the data points.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Polynomial least-squares using hyperbolic cross sets}
\label{sec:cross-sets}

Our final technique in this section for forming the approximation \eqref{eq:linear-approx} builds a polynomial approximation via least squares. In this case, the basis functions are polynomials,
\begin{linenomath}\begin{align*}
  c_k(\bxi) &= \bxi^{\alpha(k)} = \prod_{j=1}^m \left(\xi^{(j)}\right)^{\alpha(k)_j}, & \bxi &= \left( \xi^{(1)}, \ldots, \xi^{(m)}\right),
\end{align*}\end{linenomath}
where $\alpha(k) = (\alpha(k)_1, \ldots, \alpha(k)_m)\in \N_0^{m}$ is an $m$-dimensional multi-index on the non-negative integer lattice, and $\left(\alpha(k)\right)_{k=1}^K$ is any ordering of the multi-indices lying in an order-$d$ \textit{hyperbolic cross} set \cite{dung_hyperbolic_2018},
\begin{linenomath}\begin{align*}
  \left(\alpha(k)\right)_{k=1}^K \eqqcolon A = \left\{ \alpha \in \N_0^m \;\big|\; \prod_{j=1}^m (\alpha_j + 1) \leq d + 1 \right\}.
\end{align*}\end{linenomath}
Increasing the order $d$ increases the number of terms $K$ in the expansion, and hyperbolic cross sets tend to de-emphasize mixed polynomial terms and therefore have much smaller size than alternative total degree sets. Despite this decreased model capacity, polynomial approximations on hyperbolic cross sets are known to produce efficient approximations in the context of parametric PDEs \cite{dung_hyperbolic_2016,chkifa_polynomial_2018}.

We construct the coefficients $\b_k$ in \eqref{eq:linear-approx} using a weighted least squares approach on the data, and the grid is chosen as a set of weighted approximate Fekete points \cite{guo_weighted_2018}. This method is implemented with the UncertainSCI package \citep{uncertainsci}.

